The time evolution of marginally trapped surfaces

In previous work we have shown the existence of a dynamical horizon or marginally trapped tube (MOTT) containing a given strictly stable marginally outer trapped surface (MOTS). In this paper we show some results on the global behavior of MOTTs assuming the null energy condition. In particular we show that MOTSs persist in the sense that every Cauchy surface in the future of a given Cauchy surface containing a MOTS also must contain a MOTS. We describe a situation where the evolving outermost MOTS must jump during the coalescence of two seperate MOTSs. We furthermore characterize the behavior of MOTSs in the case that the principal eigenvalue vanishes under a genericity assumption. This leads to a regularity result for the tube of outermost MOTSs under the genericity assumption. This tube is then smooth up to finitely many jump times. Finally we discuss the relation of MOTSs to singularities of a space-time.

==> extern/draft_commands.tex <==
\usepackage{ifthen}

%% Collect Time and Date Info
\makeatletter
\newcommand{\pt@twodigit}[1]{{\pt@tmp=#1\relax\ifnum\pt@tmp<10 0\fi\the\pt@tmp}}
\newcount\pt@hours
\newcount\pt@minutes
\newcount\pt@tmp
\newcommand{\printtime}{%
\pt@hours=\time%
\divide\pt@hours by 60\relax%
\pt@tmp=\pt@hours%
\multiply\pt@tmp by -60\relax%
\pt@minutes=\time%
\advance\pt@minutes by \pt@tmp%
\pt@twodigit\pt@hours:\pt@twodigit\pt@minutes}

%% How to put Info in the margin
\newlength{\mt@MarginWidth}
\newlength{\mt@PageHeight}
\newlength{\mt@ActualWidth}
\newlength{\mt@MaxWidth}
\newlength{\mt@FontSize}
\newlength{\mt@RightSkip}
\newlength{\mt@TextHeight}
\newlength{\mt@OffsetX}
\newlength{\mt@OffsetY}

\usepackage{eso-pic}
\usepackage{type1cm}
\usepackage{graphicx}

\newcommand{\margintext}[1]{
  \ifx\pdfoutput\undefined\write16{WARNING: Margintext
      will only correctly show up in PS - FILE!}
  \fi
  \AddToShipoutPicture{%
    \setlength{\mt@MarginWidth}{\oddsidemargin}%
    \addtolength{\mt@MarginWidth}{1in}%
    \setlength{\mt@PageHeight}{\paperheight}%
    \setlength{\mt@MaxWidth}{.8\mt@MarginWidth}%
    \setlength{\mt@FontSize}{12mm}%
    \setlength{\mt@RightSkip}{3mm}%
    \setlength{\mt@ActualWidth}{15mm}%
    \ifthenelse{\lengthtest{\mt@ActualWidth > \mt@MaxWidth}}%
    {
      \setlength{\mt@FontSize}{.6\mt@MarginWidth}
      \setlength{\mt@RightSkip}{.2\mt@MarginWidth}
      \setlength{\mt@ActualWidth}{.8\mt@MarginWidth}
    }{}
    \setlength{\mt@OffsetX}{\mt@ActualWidth}
    \setlength{\mt@OffsetY}{0mm}
    \setlength{\unitlength}{1pt}%
    \put(\strip@pt\mt@OffsetX,\strip@pt\mt@OffsetY){%
      \rotatebox{90}
        {
          \makebox[\mt@PageHeight][c]
          {\textcolor[gray]{0.75}{\fontfamily{cmss}
              \fontseries{m}
              \fontshape{n}
              \fontsize{\mt@FontSize}{\mt@FontSize}
              \selectfont{#1}}}
        }
      }
    }
}

%% Collect information from Subversion
% If the file svn_version.tex exists, we will read it, in there
% the command \svnVersion is defined. If the file does not exist, we
% print a warning and set \svnVersion to Unknown
\newboolean{draftmargin}
\setboolean{draftmargin}{false}

\IfFileExists{draft_control.tex}{%
\message{Draft control file exists.}%
\input{draft_control.tex}%
}{% 
\message{ WARNING: draft_control.tex not found.}%
\newcommand{\svnVersion}{???}%
}


\ifthenelse{ \boolean{draftmargin} }
        {
                \margintext{Rev: {\svnVersion}\hspace{1em}Built: {\the\year-\pt@twodigit\month-\pt@twodigit\day} {\printtime}}
        }
        {}

\makeatother



==> extern/layout_commands.tex <==
\usepackage{ifthen}
\usepackage{amsmath}
\usepackage{amsthm}

\makeatletter

\newcommand{\titlefamily}{}
\newcommand{\thmfamily}{}
\newcommand{\sectitlefnt}{}
\newcommand{\subsectitlefnt}{}
\newcommand{\ps@footnumber}{}

\newcommand{\authname}[1]{#1}
\newcommand{\authaddress}[1]{#1}

%% Typesetting equations
\renewcommand{\theequation}{\arabic{section}.\arabic{equation}}
\numberwithin{equation}{section}

\newcommand{\fillbox}{\hspace*{\fill}\ensuremath{\Box}}
\renewcommand{\qedsymbol}{\fillbox}

\ifthenelse{\isundefined{\nofancylayout}}
{%
  \renewcommand{\titlefamily}{\sffamily}%
  \renewcommand{\thmfamily}{\sffamily}%
  \renewcommand{\sectitlefnt}{\titlefamily\bfseries\Large}%
  \renewcommand{\subsectitlefnt}{\titlefamily\bfseries}%
  % 
  %% Paper size and margins
  % \usepackage[shiftmargins]{vmargin}
  % \setpapersize{A4}%
  % \setmarginsrb{35mm}{25mm}{30mm}{25mm}{0mm}{0mm}{10mm}{3\baselineskip}%
  %
  \usepackage{calc}
  \usepackage[totalwidth=75ex,totalheight=41\baselineskip,vmarginratio=4:5,footskip=3\baselineskip,hcentering]{geometry}
  
  %% Typesetting the titles
  \renewcommand{\section}{\@startsection%
    {section}%
    {1}%
    {0mm}%
    {-\baselineskip}%
    {\baselineskip}%
    {\sectitlefnt}}%
  \renewcommand{\subsection}{\@startsection
    {subsection}%
    {2}%
    {0mm}%
    {-\baselineskip}%
    {0.5\baselineskip}%
    {\subsectitlefnt}}%
  \renewcommand{\ps@footnumber}{%
    \renewcommand{\@oddhead}{}%
    \renewcommand{\@evenhead}{}%
    \renewcommand{\@oddfoot}{\hfill{\thepage}}%
    \renewcommand{\@evenfoot}{{\thepage}\hfill}}

  % 
  %% Typesetting Paragraphs
  \setlength{\parskip}{1ex plus .5ex minus 0ex}
  \setlength{\parindent}{0em}
  % 
  %% Typesetting Theorems
  \newtheoremstyle{my_plain}%
  {\parskip}% above skip
  {\parskip}% below skip
  {\normalfont\itshape}% body font
  {}% indent
  {\normalfont\thmfamily\bfseries}% head font
  {.}% headpunct
  { }% headspace
  {}% custom-head-spec
  
  \newtheoremstyle{my_remark}%
  {\parskip}% aboveskip
  {\parskip}% belowskip
  {\normalfont}% bodyfont
  {}% indent
  {\normalfont\thmfamily\bfseries}% headfont
  {.}% headpunct
  { }% headspace
  {}% custom-head-spec
  
  {
    \theoremstyle{my_plain}
    \newtheorem{theorem}{Theorem}[section]
    \newtheorem{proposition}[theorem]{Proposition}
    \newtheorem{corollary}[theorem]{Corollary}
    \newtheorem{lemma}[theorem]{Lemma}
    \newtheorem{definition}[theorem]{Definition}
  }
  
  {
    \theoremstyle{my_remark}
    \newtheorem{remark}[theorem]{Remark}
  }

  \renewcommand{\authname}[1]{\titlefamily #1\hspace*{0pt}\\}
  \renewcommand{\authaddress}[1]{\begin{minipage}{.8\linewidth}\centering\titlefamily\footnotesize
      #1\hspace*{0pt}\end{minipage}\\[1ex]}
}{%
  \newtheorem{theorem}{Theorem}[section]%
  \newtheorem{proposition}[theorem]{Proposition}%
  \newtheorem{corollary}[theorem]{Corollary}%
  \newtheorem{lemma}[theorem]{Lemma}%
  \newtheorem{definition}[theorem]{Definition}%
  \theoremstyle{remark}%
  \newtheorem{remark}[theorem]{Remark}%
}

\newenvironment{abst}{\begin{quote}\small\thmfamily\bfseries
    Abstract. \normalfont\small}{\end{quote}}

\def\blfootnote{\xdef\@thefnmark{}\@footnotetext}
\makeatother

